AvatarMAV: Fast 3D Head Avatar Reconstruction Using Motion-Aware Neural Voxels

With NeRF widely used for facial reenactment, recent methods can recover photo-realistic 3D head avatar from just a monocular video. Unfortunately, the training process of the NeRF-based methods is quite time-consuming, as MLP used in the NeRF-based methods is inefficient and requires too many iterations to converge. To overcome this problem, we propose AvatarMAV, a fast 3D head avatar reconstruction method using Motion-Aware Neural Voxels. AvatarMAV is the first to model both the canonical appearance and the decoupled expression motion by neural voxels for head avatar. In particular, the motion-aware neural voxels is generated from the weighted concatenation of multiple 4D tensors. The 4D tensors semantically correspond one-to-one with 3DMM expression basis and share the same weights as 3DMM expression coefficients. Benefiting from our novel representation, the proposed AvatarMAV can recover photo-realistic head avatars in just 5 minutes (implemented with pure PyTorch), which is significantly faster than the state-of-the-art facial reenactment methods. Project page: https://www.liuyebin.com/avatarmav.

==> src/overview.tex <==
\section{Overview}

As shown in Fig.~\ref{fig:overview}, our approach reconstructs a head avatar model from a monocular portrait video. During the data preprocessing stage, we first perform 3DMM tracking to obtain the expression coefficients and head poses from the portrait video, which is used as input to our method. At the training stage of expression-related motion learning, we first establish Motion Voxel Grid (MVG) and a 2-layer MLP to represent the expression-related 3D motion. The basis of MVG share the same dimension as the 3DMM expression basis. And the same expression coefficients can be used as weights to concatenate the MVG basis. Then, at the training stage of canonical appearance reconstruction, an appearance voxel grid and another 2-layer MLP are introduced to represent the basic appearance of the target video. Specifically, given an input coordinate $x$, we then transfer it to $x+\delta x$ by MVG with the following MLP and query point $x+\delta x$ in the appearance voxel grid to get its density and color. Note that the expression coefficients and view directions are also fed into the following MLP to generate expression-related and view-dependent changes. Finally, after volumetric rendering, a consistency constraint is imposed between the rendered portrait images and the corresponding ground-truth frames. During the inference stage, we can generate photo-realistic portrait images given only expression coefficients and head poses.

%As shown in Fig.~\ref{fig:overview}, given a portrait image from training video, we first implement preprocessing to track for the expression coefficients and camera pose. Here we assume the head pose is fixed. To render a image, we preform volumetric rendering as detailed in Sec.~\ref{sec:sec:rendering}, casting rays through each pixel and sample points along each ray to query density and color. Specifically, we first compute the motion voxel grid by concatenating the multiple neural voxel grids basis with tracked 3DMM expression coefficients as corresponding weights. Then given a point in world space, we query its offset through the motion voxel grid to transform the point to canonical space. Finally, we query density and color through the appearance voxel grid as detailed in Sec.~\ref{sec:sec:representation}. At training stage, we use input image with area outside the face removed for supervision.
